One Masked Model is All You Need for Sensor Fault Detection, Isolation and Accommodation

Accurate and reliable sensor measurements are critical for ensuring the safety and longevity of complex engineering systems such as wind turbines. In this paper, we propose a novel framework for sensor fault detection, isolation, and accommodation (FDIA) using masked models and self-supervised learning. Our proposed approach is a general time series modeling approach that can be applied to any neural network (NN) model capable of sequence modeling, and captures the complex spatio-temporal relationships among different sensors. During training, the proposed masked approach creates a random mask, which acts like a fault, for one or more sensors, making the training and inference task unified: finding the faulty sensors and correcting them. We validate our proposed technique on both a public dataset and a real-world dataset from GE offshore wind turbines, and demonstrate its effectiveness in detecting, diagnosing and correcting sensor faults. The masked model not only simplifies the overall FDIA pipeline, but also outperforms existing approaches. Our proposed technique has the potential to significantly improve the accuracy and reliability of sensor measurements in complex engineering systems in real-time, and could be applied to other types of sensors and engineering systems in the future. We believe that our proposed framework can contribute to the development of more efficient and effective FDIA techniques for a wide range of applications.

==> figures/figure_2_inference.tex <==
\begin{figure}
  \centering
    \begin{subfigure}[b]{1.0\linewidth}
      \begin{equation*}
      \begin{aligned}
        \left[
        \begin{aligned}
          \hat{x^1}\\[-0.5em]
          \rule{1em}{1em}\\[-0.5em]
          \rule{1em}{1em}\\[-1em]
          \vdots\\[-0.5em]
          \rule{1em}{1em}
        \end{aligned}
        \right]_{t, t-1, t-2, ...} &= f\left(
        \left[
        \begin{aligned}
          \rule{1em}{1em}\\[-0.5em]
          x^2\\[-0.5em]
          x^3\\[-1em]
          \vdots\\[-0.5em]
          x^n
        \end{aligned}
        \right]_{t, t-1, t-2, ...}
        \right),
        \\
        \left[
          \begin{aligned}
            \rule{1em}{1em}\\[-0.5em]
            \hat{x^2}\\[-0.5em]
            \rule{1em}{1em}\\[-1em]
            \vdots\\[-0.5em]
            \rule{1em}{1em}
          \end{aligned}
          \right]_{t, t-1, t-2, ...} &= f\left(
          \left[
          \begin{aligned}
            x^1\\[-0.5em]
            \rule{1em}{1em}\\[-0.5em]
            x^3\\[-1em]
            \vdots\\[-0.5em]
            x^n
          \end{aligned}
          \right]_{t, t-1, t-2, ...}
        \right),
        \\
        \cdots,  
        \\
        \left[
        \begin{aligned}
          \rule{1em}{1em}\\[-0.5em]
          \rule{1em}{1em}\\[-0.5em]
          \rule{1em}{1em}\\[-1em]
          \vdots\\[-0.5em]
          \hat{x^n}
        \end{aligned}
        \right]_{t, t-1, t-2, ...} &= f\left(
        \left[
        \begin{aligned}
          x^1\\[-0.5em]
          x^2\\[-0.5em]
          x^3\\[-1em]
          \vdots\\[-0.5em]
          \rule{1em}{1em}
        \end{aligned}
        \right]_{t, t-1, t-2, ...}
        \right)
      \end{aligned}
      \end{equation*}
      % \vspace{-8pt}
      \caption{Step 1: Sequentially mask each channel and calculate predictions for that channel using information from all other sensors.}
      \label{fig:inference:subfig1}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
      \begin{equation*}
        x^i = 
        \begin{cases} 
        \hat{x^i} & \lvert\hat{x^i}-x^i\rvert>\theta_i \\
        x^i & \text{otherwise} 
        \end{cases} \quad \text{for } i = 1, 2, \dots, n
      \end{equation*}
      % \vspace{-8pt}
      \caption{Step 2: Sensor fault detection, isolation, and accommodation. For each channel $i$, we compare the residual between the sensor data $x^i$ and the model's prediction $\hat{x^i}$ to a threshold $\theta_i$. If the residual is larger than $\theta_i$, there is a fault at sensor $i$, and we replace the sensor data with the model's prediction. Otherwise, the sensor data is kept unchanged.}
      \label{fig:inference:subfig2}
    \end{subfigure}
  \caption{Inference scheme for our proposed masked method.}
  \label{fig:inference}
\end{figure}

